The noise level in linear regression with dependent data

We derive upper bounds for random design linear regression with dependent ($\beta$-mixing) data absent any realizability assumptions. In contrast to the strictly realizable martingale noise regime, no sharp instance-optimal non-asymptotics are available in the literature. Up to constant factors, our analysis correctly recovers the variance term predicted by the Central Limit Theorem -- the noise level of the problem -- and thus exhibits graceful degradation as we introduce misspecification. Past a burn-in, our result is sharp in the moderate deviations regime, and in particular does not inflate the leading order term by mixing time factors.

==> notes.tex <==

To appreciate the above statement, let us simplify the theorem. Let $|O| \sim |E|$ and note that we may then upper-bound:
\begin{equation}
    \max_{\sgn\in \{O,E \}} \sqrt{\frac{\Lambda_{\sgn}}{|\sgn|}} \lesssim   \sqrt{\frac{\Lambda}{n}}. 
\end{equation}
If further $(\sfZ, \|\cdot\|) = (\R^d, \|\cdot\|_2)$ we have $r \leq d$. Hence for some constants $c,c'>0$:
 \begin{multline}
      \mathbf{P} \left( \left\|\frac{1}{n}\sum_{i=1}^n Z_i\right\| \geq  c \sqrt{\frac{\Lambda}{n}}\left(\sqrt{d}  
+
\sqrt{ \log (1/\delta)}\right) \right)\\
\leq 2\delta+  \sum_{i=2}^{2m-1} \beta_Z(a_i)
 +
\frac{(c')^s}{d^{s/2}{n}^{s/2}}  \sum_{a_i \subset [n]} \frac{\E \left\| \sum_{j\in a_i} Z_j \right\|^s}{\Lambda^{s/2}}.
\end{multline}
Hence as long the burn-in holds:
\begin{equation}
    n \geq c'' d^{-1} \left(\frac{1}{\delta} \right)^{s/2} \left( \sum_{a_i \subset [n]} \frac{\E \left\| \sum_{j\in a_i} Z_j \right\|^s}{\Lambda^{s/2}}\right)^{2/s} \textnormal{ and }  \sum_{i=2}^{2m-1} \beta_Z(a_i) \leq \delta.
\end{equation}
we have:
\begin{equation}
      \mathbf{P} \left( \left\|\frac{1}{n}\sum_{i=1}^n Z_i\right\| \geq  c \sqrt{\frac{\Lambda}{n}}\left(\sqrt{d}  
+
\sqrt{ \log (4/\delta)}\right) \right)
\leq \delta
\end{equation}

Next, it also worth to point out that if the process is stationary and $|E|=|O|$ we have
\begin{equation*}
    \Lambda_{E} = \Lambda_{O} \quad \textnormal{and also}\quad
     \Lambda_{E} + \Lambda_{O} = 2 \Lambda 
\end{equation*}
so our analysis is always loose by a factor $\sqrt{2}$.

It is also worth to point out that if the $Z_j$ are $1$-bounded in $\|\cdot \|$, then $\E \left\| \sum_{j\in a_i} Z_j \right\|^s \leq | a_i|^s$ by the triangle inequality. This informs us about how many moments we need. For $n^\alpha$ blocks of size $n^{1-\alpha}$ we require 
\begin{equation}
    n^\alpha n^{(1-\alpha)s} = o(n^{s/2}) \Leftrightarrow s > \frac{2\alpha}{1-2(1-\alpha)} = \frac{2\alpha}{2\alpha -1}
\end{equation}
and  we always must have $\alpha >1/2$ - we need at least $\sqrt{n}$ many blocks. The interpretation above is that the fewer blocks we have $\alpha \to 1/2$ the more moments we require.

We also have a second constraint on $\alpha$ since we need
\begin{equation}
    n^{\alpha} \beta(n^{1-\alpha}) = o(1)
\end{equation}
for $\beta(a) = (a)^{-q}$ this implies
\begin{equation}
     n^{\alpha} \frac{1}{n^{q(1-\alpha)}} = o(1)
\end{equation}
so that $q >\alpha /(1-\alpha)$. The more blocks we have (increasing $\alpha$)  the faster the mixing rate $q$ needs to be.

